Empowering Mobile Networks Security Resilience by using Post-Quantum Cryptography

The transition to a cloud-native 5G Service-Based Architecture (SBA) improves scalability but exposes control-plane signaling to emerging quantum threats, including Harvest-Now, Decrypt-Later (HNDL) attacks. While NIST has standardized post-quantum cryptography (PQC), practical, deployable integration in operational 5G cores remains underexplored. This work experimentally integrates NIST-standardized ML-KEM-768 and ML-DSA into an open-source 5G core (free5GC) using a sidecar proxy pattern that preserves unmodified network functions (NFs). Implemented on free5GC, we compare three deployments: (i) native HTTPS/TLS, (ii) TLS sidecar, and (iii) PQC-enabled sidecar. Measurements at the HTTP/2 request-response boundary over repeated independent runs show that PQC increases end-to-end Service-Based Interface (SBI) latency to approximately 54 ms, adding a deterministic 48-49 ms overhead relative to the classical baseline, while maintaining tightly bounded variance (IQR <= 0.2 ms, CV < 0.4%). We also quantify the impact of Certification Authority (CA) security levels, identifying certificate validation as a tunable contributor to overall delay. Overall, the results demonstrate that sidecar-based PQC insertion enables a non-disruptive and operationally predictable migration path for quantum-resilient 5G signaling.

==> paper/acronym.tex <==
%Numbering
\acrodef{3GPP}{3rd Generation Partnership Project}
\acrodef{5G}{5th Generation Mobile Network}
\acrodef{6G}{6th Generation Mobile Network}
%-----A-----
\acrodef{AI}{Artificial Intelligence}
\acrodef{AI4Net}{\ac{AI} for Networking}
\acrodef{AIDER}{Aerial Image Dataset for Emergency Response}
\acrodef{AIaaS}{Artificial Intelligence-as-a-Service}
\acrodef{AMF}{Access and Mobility Management Function}
\acrodef{API}{Application Programming Interface}
\acrodef{AUSF}{Authentication Server Function}
\acrodef{IID}{Independent and Identically Distributed}
%-----B----- 
\acrodef{B5G}{Beyond Fifth Generation}
\acrodef{BPF}{Berkeley Packet Filter}
%-----C-----
\acrodef{CA}{Certificate Authority}
\acrodef{CBR}{Constant Bit Rate}
\acrodef{CI}{Confidence Interval}
\acrodef{CV}{Coefficient of Variation}
\acrodef{CSV}{Comma-Separated Values}
\acrodef{CPU}{Central Processing Unit}
\acrodef{CNN}{Convolutional Neural Network}
\acrodef{CNNs}{Convolutional Neural Networks}
\acrodef{CRQC}{Cryptographically Relevant Quantum Computer}

%-----D-----
\acrodef{DCA}{Dynamic Cryptographic Agility}
\acrodef{DoS}{Denial of Service}
\acrodef{DDoS}{Distributed Denial of Service}
\acrodef{DDPG}{Deep Deterministic Policy Gradient}
\acrodef{DNN}{Deep Neural Network}
\acrodef{DSA}{Digital Signature Algorithms}
\acrodef{DRL}{Deep Reinforcement Learning}
\acrodef{DT}{Decision Tree}

%-----E-----
\acrodef{ETSI}{European Telecommunications Standards Institute}
\acrodef{eNWDAF}{Evolved Network Data Analytics Function}
\acrodef{ECC}{Elliptic-curve cryptography}
\acrodef{E2E}{End-To-End}

%-----F-----
\acrodef{FIBRE}{Future Internet Brazilian Environment for Experimentation}
\acrodef{Fuzz}{(Fuzzing or Fuzz testing) - Automated Software Testing Technique}

%-----G-----
\acrodef{GNN}{Graph Neural Networks}
\acrodef{GPU}{Graphics Processing Unit}
%-----H-----
\acrodef{HTM}{Hierarchical Temporal Memory}
\acrodef{HNDL}{Harvest Now, Decrypt Later}
\acrodef{HTTP}{Hypertext Transfer Protocol}
\acrodef{HTTPS}{Hypertext Transfer Protocol Security}
\acrodef{HSM}{Hardware Security Module}


%-----I----- 
\acrodef{IAM}{Identity And Access Management}
\acrodef{ICMP}{Internet Control Message Protocol}
\acrodef{IID}{Informally, Identically Distributed}
\acrodef{IoE}{Internet of Everything}
\acrodef{IoT}{Internet of Things}
\acrodef{IQR}{Interquartile Range}
\acrodef{IPsec}{Internet Protocol Security}
\acrodef{ITU}{International Telecommunication Union}
%-----J-----
%-----K-----
\acrodef{KEM}{Key Encapsulation Mechanism}
\acrodef{KNN}{K-Nearest Neighbors}
\acrodef{KPI}{Key Performance Indicator}
\acrodef{KPIs}{Key Performance Indicators}
%-----L-----
\acrodef{LSTM}{Long Short-Term Memory}
\acrodef{LTS}{Long Term Support }

%-----M----- 
\acrodef{MITM}{Man-in-the-Middle}
\acrodef{MAE}{Mean Absolute Error}
\acrodef{MACsec}{Media Access Control Security}
\acrodef{ML}{Machine Learning}
\acrodef{MLaaS}{Machine Learning as a Service}
\acrodef{MOS}{Mean Opinion Score}
\acrodef{MAPE}{Mean Absolute Percentage Error}
\acrodef{MSE}{Mean Squared Error}
\acrodef{MEC}{Multi-access Edge Computing}
\acrodef{mMTC}{Massive Machine Type Communications}
\acrodef{MFA}{Multi-factor Authentication}

%-----N-----
\acrodef{NWDAF}{Network Data Analytics Function}
\acrodef{NSSF}{Network Slice Selection Function}
\acrodef{Net4AI}{Networking for \ac{AI}}
\acrodef{NIST}{National Institute of Standards and Technology}
\acrodef{NS}{Network Slicing}
\acrodef{NF}{Network Function}
\acrodef{NFV}{Network Function Virtualization}
\acrodef{NFVM}{Network Function Virtualization Management}
\acrodef{NRF}{Network Repository Function}
  
%-----O----- 
\acrodef{OSM}{Open Source MANO}
\acrodef{OAuth}{Open Authorization}
\acrodef{OQS}{Open Quantum Safe}

%-----P-----
\acrodef{PCA}{Principal Component Analysis}
\acrodef{PDU}{Packet Data Unit}
\acrodef{PCF}{Policy Control Function}
\acrodef{PoC}{Proof of Concept}
\acrodef{PQC}{Post-Quantum Cryptography }
%\acrodef{PQC-Proxy}{\ac{PQC} Proxy}

%-----Q-----
\acrodef{QoE}{Quality of experience}
\acrodef{QoS}{Quality of Service}

%-----R-----
\acrodef{RAM}{Random Access Memory}
\acrodef{RESTful}{REpresentational State Transfer Application Programming Interface}
\acrodef{RF}{Random Forest}
\acrodef{RL}{Reinforcement Learning}
\acrodef{RMSE}{Root Mean Square Error}
\acrodef{RNN}{Recurrent Neural Network}
\acrodef{RTT}{Round-Trip Time}
\acrodef{RAN}{Radio Access Network}
\acrodef{RSA}{Rivest–Shamir–Adleman}
\acrodef{RX}{Receive}
%-----S-----   
\acrodef{SBA}{Service-Based Architecture}
\acrodef{SBI}{Service-Based Interface}
\acrodef{SCTP}{Stream Control Transmission Protocol}
\acrodef{SDN}{Software-Defined Networking}
\acrodef{SFI2}{Slicing Future Internet Infrastructures}
\acrodef{SLA}{Service-Level Agreement}
\acrodef{SON}{Self-Organizing Network}
\acrodef{SMF}{Session Management Function}
\acrodef{S-NSSAI}{Single Network Slice Selection Assistance Information}
\acrodef{SPPQC}{Sidecar Proxy \ac{PQC}}
\acrodef{SVM}{Support Vector Machine}

%-----T-----   
\acrodef{TCP}{Transmission Control Protocol}
\acrodef{TEE}{Trusted Execution Environment}
\acrodef{TQFL}{Trust Deep Q-learning Federated Learning}
\acrodef{TLS}{Transport Layer Security}
%\acrodef{TLS-Proxy}{\ac{TLS} Proxy}
\acrodef{TLSSP}{\ac{TLS} Sidecar Proxy}
\acrodef{TEID}{Tunnel Endpoint Identifier}
\acrodef{TX}{Transmit}

%-----U----- 
\acrodef{UE}{User Equipment}
\acrodef{UDM}{Unified Data Management}
\acrodef{UPF}{User Plane Function}
\acrodef{UDR}{Unified Data Repository}
\acrodef{URLLC}{Ultra-Reliable and Low Latency Communications}
\acrodef{UAV}{Unmanned Aerial Vehicle}
\acrodef{UAVs}{Unmanned Aerial Vehicles}

%-----V-----
\acrodef{VoD}{Video on Demand}
\acrodef{VM}{Virtual Machine}
\acrodef{VR}{Virtual Reality}
\acrodef{AR}{Augmented Reality}
\acrodef{V2V}{Vehicle-to-Vechile}
\acrodef{V2X}{Vehicle-to-Everything}


%-----W-----
%-----X-----
%-----Y-----
%-----Z-----
